Snap Video: Scaled Spatiotemporal Transformers for Text-to-Video Synthesis

Contemporary models for generating images show remarkable quality and versatility. Swayed by these advantages, the research community repurposes them to generate videos. Since video content is highly redundant, we argue that naively bringing advances of image models to the video generation domain reduces motion fidelity, visual quality and impairs scalability. In this work, we build Snap Video, a video-first model that systematically addresses these challenges. To do that, we first extend the EDM framework to take into account spatially and temporally redundant pixels and naturally support video generation. Second, we show that a U-Net - a workhorse behind image generation - scales poorly when generating videos, requiring significant computational overhead. Hence, we propose a new transformer-based architecture that trains 3.31 times faster than U-Nets (and is ~4.5 faster at inference). This allows us to efficiently train a text-to-video model with billions of parameters for the first time, reach state-of-the-art results on a number of benchmarks, and generate videos with substantially higher quality, temporal consistency, and motion complexity. The user studies showed that our model was favored by a large margin over the most recent methods. See our website at https://snap-research.github.io/snapvideo/.

==> figures/architecture.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{resources/architecture.pdf}
  \caption{Architecture of our proposed FIT. Given noisy input video $\xx_{\sigmanoise}$, the model estimates the denoised video $\xxh_{\sigmanoise}$ by recurrent application of FIT blocks. Each block reads information from the patch tokens into a small set of latent tokens on which computation is performed. The results, are written to the patch tokens. Conditioning information in the form of text embeddings, noise level $\sigma$, framerate $\framerate$ and resolution $\resolution$ is provided through an additional read operation.}
  \label{fig:architecture}
\end{figure}

==> figures/spatiotemporal_computation.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{resources/spatiotemporal_computation.pdf}
  \caption{Architecture of our proposed FIT. Given noisy input video $\xx_{\sigmanoise}$, the model estimates the denoised video $\xxh_{\sigmanoise}$ by recurrent application of FIT blocks. Each block reads information from the patch tokens into a small set of latent tokens on which computation is performed. The results, are written to the patch tokens. Conditioning information in the form of text embeddings, noise level $\sigma$, framerate $\framerate$ and resolution $\resolution$ is provided through an additional read operation.}
  \label{fig:spatiotemporal_computation}
\end{figure}


==> sections/equations_edm_is_a_v_prediction_framework.tex <==
We derive the effective training target of EDM
\begin{eqnarray}
  \mathcal{L}(\netd) &=& \mathbb{E}_{\sigmanoise \sim \ptrain} \big[ \lambda(\sigmanoise) ~\mathcal{L}(\netd; \sigmanoise) \big] \\
  &=& \mathbb{E}_{\sigmanoise \sim \ptrain} ~\Big[ \lambda(\sigmanoise) ~\mathbb{E}_{\xx \sim \pdata} ~\mathbb{E}_{\noise \sim \mathcal{N}(\boldzero, \boldi)} ~\big\lVert \netd(\xx + \sigmanoise \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise \sim \ptrain} ~\mathbb{E}_{\xx \sim \pdata} ~\mathbb{E}_{\noise \sim \mathcal{N}(\boldzero, \sigmanoise^2 \boldi)}  ~\Big[ \lambda(\sigmanoise) ~\big\lVert \netd(\xx + \sigmanoise \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) ~\big\lVert \netd(\xx + \sigmanoise \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big]
  \text{,}
\end{eqnarray}

We insert the definition of $\netd$
\begin{eqnarray}
  && \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \cskip(\sigmanoise) (\xx {+} \sigmanoise \noise) + \cout(\sigmanoise) \netf\big(\Fargs\big) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \cout(\sigmanoise) \netf\big(\Fargs\big) - \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise \noise) \big) \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \cout(\sigmanoise)^2 \big\lVert \netf\big(\Fargs\big) - \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx {+} \sigmanoise \noise) \big) \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ w(\sigmanoise) ~\big\lVert \netf\big(\Fargs\big) - F_\text{target}(\xx, \noise; \sigmanoise) \big\rVert^2_2 \Big]
  \text{,}
\end{eqnarray}

Effective training target
\begin{equation}
  F_\text{target}(\xx, \noise; \sigmanoise) = \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise \noise) \big)
  \text{,}
\end{equation}

Also we have that
\begin{eqnarray}
  \cin(\sigmanoise) &=& 1 \big/ \sqrt{\sigmanoise^2 + \sigmadata^2}
  \text{.}
\end{eqnarray}

\begin{eqnarray}
  \cout(\sigmanoise) &=& \sigmanoise \cdot \sigmadata \big/ \sqrt{\sigmanoise^2 + \sigmadata^2}
  \text{.}
\end{eqnarray}

\begin{eqnarray}
  \cskip(\sigmanoise) &=& \sigmadata^2 / \big( \sigmanoise^2 + \sigmadata^2 \big)
  \text{.}
\end{eqnarray}

Substituting $\cskip$ and $\cout$ we obtain
\begin{eqnarray}
  F_\text{target}(\xx, \noise; \sigmanoise) &=& \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise \noise) \big) \\
  &=& \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \frac{\sigmadata^2}{\big( \sigmanoise^2 + \sigmadata^2 \big)} (\sigmanoise) (\xx + \sigmanoise \noise) \big) \\
  &=& \tfrac{1}{\cout(\sigmanoise)} \big( \xx \left( \frac{\sigmanoise^2}{\sigmanoise^2 + \sigmadata^2} \right)  - \frac{\sigmadata^2}{\big( \sigmanoise^2 + \sigmadata^2 \big)} \sigmanoise \noise \big) \\
  &=& \tfrac{1}{\cout(\sigmanoise)} \left( \frac{\sigmanoise}{\sigmanoise^2 + \sigmadata^2} \right)  \big( \sigmanoise \xx - \sigmadata^2 \noise \big)  \\
  &=& \tfrac{1}{\sqrt{\sigmanoise^2 + \sigmadata^2} \sigmadata} \big( \sigmanoise \xx - \sigmadata^2 \noise \big)  \\
  \text{,}
\end{eqnarray}

Substituting $\sigmadata=1$ we obtain
\begin{eqnarray}
  F_\text{target}(\xx, \noise; \sigmanoise) &=& \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise \noise) \big) \\
  &=& \tfrac{1}{\sqrt{\sigmanoise^2 + \sigmadata^2} \sigmadata} \big( \sigmanoise \xx - \sigmadata^2 \noise \big)  \\
  \text{,}
&=& \tfrac{1}{\sqrt{\sigmanoise^2 + 1}} \big( \sigmanoise \xx - \noise \big)  \\
  \text{,}
\end{eqnarray}
which is the v prediction objective with a normalization factor equal to the standard deviation.

From EDM we also have
\begin{eqnarray}
  \lossweight(\sigmanoise) &=& \tfrac{1}{\cout(\sigmanoise)^2} \\
  &=& \frac{\sigmanoise^2 + \sigmadata^2}{\big(\sigmanoise \sigmadata\big)^2} \\
  &=& \frac{1}{\sigmadata^2} + \frac{1}{\sigmanoise^2} \\
\end{eqnarray}

Where by substituting $\sigmadata=1$ we obtain
\begin{eqnarray}
  \lossweight(\sigmanoise) &=& \tfrac{1}{\cout(\sigmanoise)^2} \\
  &=& 1 + \frac{1}{\sigmanoise^2} \\
  &=& 1 + \text{SNR} \\
\end{eqnarray}
which is the v prediction loss weighting.

We see that $\sigmadata$ acts in two ways on the definition of the diffusion framework. First, by introducing a constant factor in the definition of v. Second, by introducing a weighting factor in the loss weighting.

==> sections/equations_edm_original.tex <==

Overall training objective EDM part 1
\begin{equation}
  \mathcal{L}(\netd; \sigmanoise) = \mathbb{E}_{\xx \sim \pdata} ~\mathbb{E}_{\noise \sim \mathcal{N}(\boldzero,  \boldi)} ~\big\lVert \netd(\xx + \sigmanoise * \noise; \sigmanoise) - \xx \big\rVert^2_2
  \text{.}
\end{equation}

Overall training objective EDM part 2
\begin{eqnarray}
  \mathcal{L}(\netd) &=& \mathbb{E}_{\sigmanoise \sim \ptrain} \big[ \lambda(\sigmanoise) ~\mathcal{L}(\netd; \sigmanoise) \big] \\
  &=& \mathbb{E}_{\sigmanoise \sim \ptrain} ~\Big[ \lambda(\sigmanoise) ~\mathbb{E}_{\xx \sim \pdata} ~\mathbb{E}_{\noise \sim \mathcal{N}(\boldzero, \sigmanoise^2 \boldi)} ~\big\lVert \netd(\xx + \sigmanoise * \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise \sim \ptrain} ~\mathbb{E}_{\xx \sim \pdata} ~\mathbb{E}_{\noise \sim \mathcal{N}(\boldzero, \sigmanoise^2 \boldi)}  ~\Big[ \lambda(\sigmanoise) ~\big\lVert \netd(\xx + \sigmanoise * \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) ~\big\lVert \netd(\xx + \sigmanoise * \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big]
  \label{eq:totalloss}
  \text{,}
\end{eqnarray}

Derivation of effective training target EDM
\begin{eqnarray}
  && \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \cskip(\sigmanoise) (\xx {+} \sigmanoise * \noise) + \cout(\sigmanoise) \netf\big(\Fargs\big) - \xx \big\rVert^2_2 \Big] \label{eq:lossexpanded} \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \cout(\sigmanoise) \netf\big(\Fargs\big) - \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise * \noise) \big) \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \cout(\sigmanoise)^2 \big\lVert \netf\big(\Fargs\big) - \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx {+} \sigmanoise * \noise) \big) \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ w(\sigmanoise) ~\big\lVert \netf\big(\Fargs\big) - F_\text{target}(\xx, \noise; \sigmanoise) \big\rVert^2_2 \Big]
  \text{,}
\end{eqnarray}

Effective training target
\begin{equation}
  F_\text{target}(\xx, \noise; \sigmanoise) = \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise * \noise) \big)
  \text{,}
\end{equation}


Derivation of cin EDM
\begin{eqnarray}
  \Var_{\xx, \noise} \big[ \cin(\sigmanoise) (\xx + \sigmanoise * \noise) \big] &=& 1 \\
  \cin(\sigmanoise)^2 ~\Var_{\xx, \noise} \big[ \xx + \sigmanoise * \noise \big] &=& 1 \\
  \cin(\sigmanoise)^2 \big( \sigmadata^2 + \sigmanoise^2 \big) &=& 1 \\
  \cin(\sigmanoise) &=& 1 \big/ \sqrt{\sigmanoise^2 + \sigmadata^2}
  \text{.}
\end{eqnarray}

Derivation of cout EDM part 1
\begin{eqnarray}
  \Var_{\xx, \noise} \big[ F_\text{target}(\xx, \noise; \sigmanoise) \big] &=& 1 \\
  \Var_{\xx, \noise} \Big[ \tfrac{1}{\cout(\sigmanoise)} \big( \xx - \cskip(\sigmanoise) (\xx + \sigmanoise * \noise) \big) \Big] &=& 1 \\
  \tfrac{1}{\cout(\sigmanoise)^2} \Var_{\xx, \noise} \big[ \xx - \cskip(\sigmanoise) (\xx + \sigmanoise * \noise) \big] &=& 1 \\
  \cout(\sigmanoise)^2 &=& \Var_{\xx, \noise} \big[ \xx - \cskip(\sigmanoise) (\xx + \sigmanoise * \noise) \big] \\
  \cout(\sigmanoise)^2 &=& \Var_{\xx, \noise} \Big[ \big( 1 - \cskip(\sigmanoise) \big) ~\xx + \cskip(\sigmanoise) ~\noise \Big] \\
  \cout(\sigmanoise)^2 &=& \big( 1 - \cskip(\sigmanoise) \big)^2 ~\sigmadata^2 + \cskip(\sigmanoise)^2 ~\sigmanoise^2
  \label{eq:coutpre}
  \text{.}
\end{eqnarray}

Derivation of cskip EDM
\begin{eqnarray}
  0 &=& \diff\big[ \cout(\sigmanoise)^2 \big] / \diff\cskip(\sigmanoise) \\
  0 &=& \diff\Big[ \big(1 - \cskip(\sigmanoise)\big)^2 ~\sigmadata^2 + \cskip(\sigmanoise)^2 ~\sigmanoise^2 \Big] / \diff\cskip(\sigmanoise) \\
  0 &=& \sigmadata^2 ~\diff \Big[ \big(1 - \cskip(\sigmanoise)\big)^2 \Big] / \diff\cskip(\sigmanoise) + \sigmanoise^2 ~\diff\big[\cskip(\sigmanoise)^2 \big] / \diff \cskip(\sigmanoise) \\
  0 &=& \sigmadata^2 ~\big[ 2 ~\cskip(\sigmanoise) - 2 \big] + \sigmanoise^2 ~\big[ 2 ~\cskip(\sigmanoise) \big] \\
  0 &=& \big( \sigmanoise^2 + \sigmadata^2 \big) ~\cskip(\sigmanoise) - \sigmadata^2 \\
  \cskip(\sigmanoise) &=& \sigmadata^2 / \big( \sigmanoise^2 + \sigmadata^2 \big)
  \label{eq:cskip}
  \text{.}
\end{eqnarray}

Derivation of cout EDM part 2
\begin{eqnarray}
  \cout(\sigmanoise)^2 &=& \big( 1 - \big[ \cskip(\sigmanoise) \big] \big)^2 ~\sigmadata^2 + \big[ \cskip(\sigmanoise) \big]^2 ~\sigmanoise^2 \\
  \cout(\sigmanoise)^2 &=& \bigg( 1 - \bigg[ \frac{\sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \bigg] \bigg)^2 ~\sigmadata^2 + \bigg[ \frac{\sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \bigg]^2 ~\sigmanoise^2 \\
  \cout(\sigmanoise)^2 &=& \bigg[ \frac{\sigmanoise^2 ~\sigmadata}{\sigmanoise^2 + \sigmadata^2} \bigg]^2 + \bigg[ \frac{\sigmadata^2 ~\sigmanoise}{\sigmanoise^2 + \sigmadata^2} \bigg]^2 \\
  \cout(\sigmanoise)^2 &=& \frac{\big( \sigmanoise^2 ~\sigmadata \big)^2 + \big( \sigmadata^2 ~\sigmanoise \big)^2}{\big( \sigmanoise^2 + \sigmadata^2 \big)^2} \\
  \cout(\sigmanoise)^2 &=& \frac{(\sigmanoise \cdot \sigmadata)^2 ~\big( \sigmanoise^2 + \sigmadata^2 \big)}{\big( \sigmanoise^2 + \sigmadata^2 \big)^2} \\
  \cout(\sigmanoise)^2 &=& \frac{(\sigmanoise \cdot \sigmadata)^2}{\sigmanoise^2 + \sigmadata^2} \\
  \cout(\sigmanoise) &=& \sigmanoise \cdot \sigmadata \big/ \sqrt{\sigmanoise^2 + \sigmadata^2}
  \text{.}
\end{eqnarray}

Derivation of loss weight EDM
\begin{eqnarray}
  w(\sigmanoise) &=& 1 \\
  \lambda(\sigmanoise) ~\cout(\sigmanoise)^2 &=& 1 \\
  \lambda(\sigmanoise) &=& 1 / \cout(\sigmanoise)^2 \\
  \lambda(\sigmanoise) &=& 1 \big/ \bigg[ \frac{\sigmanoise \cdot \sigmadata}{\sqrt{\sigmanoise^2 + \sigmadata^2}} \bigg]^2 \\
  \lambda(\sigmanoise) &=& 1 \big/ \bigg[ \frac{(\sigmanoise \cdot \sigmadata)^2}{\sigmanoise^2 + \sigmadata^2} \bigg] \\
  \lambda(\sigmanoise) &=& \big( \sigmanoise^2 + \sigmadata^2 \big) / (\sigmanoise \cdot \sigmadata)^2
  \text{.}
\end{eqnarray}

==> sections/equations_edm_with_naive_input_scaling.tex <==
We derive the effective training target of EDM where we introduce the input scaling factor $\sigmain$
\begin{eqnarray}
  \mathcal{L}(\netd) &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) ~\big\lVert \netd(\frac{\xx}{\sigmain} + \sigmanoise \noise; \sigmanoise) - \xx \big\rVert^2_2 \Big]
  \text{,}
\end{eqnarray}

We insert the definition of $\netd$
\begin{eqnarray}
  && \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \cskip(\sigmanoise) (\frac{\xx}{\sigmain} {+} \sigmanoise \noise) + \cout(\sigmanoise) \netf\big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \big\lVert \frac{\sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) + \frac{\sigmanoise \sigmadata}{\sqrt{\sigmanoise^2 + \sigmadata^2}} \netf\big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) - \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \frac{\sigmanoise^2 \sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \big\lVert \frac{\sigmadata}{\sigmanoise \sqrt{\sigmanoise^2 + \sigmadata^2}} \big(\frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) + \netf\big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) - \frac{\sqrt{\sigmanoise^2 + \sigmadata^2}}{\sigmanoise \sigmadata} \xx \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \frac{\sigmanoise^2 \sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \big\lVert \netf\big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) - \frac{\sigmadata^2 (\xx - \frac{\xx}{\sigmain}) + \sigmanoise^2 \xx - \sigmanoise \sigmadata^2 \noise}{\sigmanoise \sigmadata \sqrt{\sigmanoise^2 + \sigmadata^2}} \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lambda(\sigmanoise) \frac{\sigmanoise^2 \sigmadata^2}{\sigmanoise^2 + \sigmadata^2} \big\lVert \netf\big( \frac{\xx}{\sigmain} {+} \sigmanoise \noise \big) - \frac{\sigmadata}{\sigmanoise \sqrt{\sigmanoise^2 + \sigmadata^2}} (\xx - \frac{\xx}{\sigmain}) - \frac{\sigmanoise \xx - \sigmadata^2 \noise}{\sigmadata \sqrt{\sigmanoise^2 + \sigmadata^2}} \big\rVert^2_2 \Big] \\
  \text{,}
\end{eqnarray}
Where the training target has a spurious term $\frac{\sigmadata}{\sigmanoise \sqrt{\sigmanoise^2 + \sigmadata^2}} (\xx - \frac{\xx}{\sigmain})$ which approaches infinity as $\sigmanoise$ approaches 0.

==> sections/equations_our_framework.tex <==

Formulation of our training target
\begin{equation}
  F_\text{target}(\xx, \noise; \sigmanoise) = \tfrac{1}{\cout(\sigmanoise)} \big( \sigmadata^2 \noise - \sigmanoise \xx \big)
  \text{,}
\end{equation}


As in EDM we require the effective training target $F_\text{target}$ to have unit variance:
\begin{eqnarray}
  \Var_{\xx, \noise} \big[ F_\text{target}(\xx, \noise; \sigmanoise) \big] &=& 1 \\
  \Var_{\xx, \noise} \Big[ \tfrac{1}{\cout(\sigmanoise)} \big( \sigmadata^2 \noise - \sigmanoise \xx \big) \Big] &=& 1 \\
  \Var_{\xx, \noise} \Big[ \big( \sigmadata^2 \noise - \sigmanoise \xx \big) \Big] &=& \cout(\sigmanoise)^2 \\
  \cout(\sigmanoise)^2 &=& \sigmadata^2 (\sigmadata^2 + \sigmanoise^2) \\
  \cout(\sigmanoise) &=& \sqrt{\sigmadata^2 (\sigmadata^2 + \sigmanoise^2)} \\
  \text{.}
\end{eqnarray}

As in EDM we require the model input to have unit variance:
\begin{eqnarray}
  \Var_{\xx, \noise} \big[ \frac{1}{\cin(\sigmanoise)} (\frac{\xx}{\sigmain} + \sigmanoise \noise) \big] &=& 1 \\
  \Var_{\xx, \noise} \big[ \frac{\xx}{\sigmain} + \sigmanoise \noise \big] &=& \cin(\sigmanoise)^2 \\
  \cin(\sigmanoise)^2 &=& \frac{\sigmadata^2}{\sigmain^2} + \sigmanoise^2\\
  \cin(\sigmanoise) &=& \sqrt{\frac{\sigmadata^2}{\sigmain^2} + \sigmanoise^2}\\
  \text{.}
\end{eqnarray}


We define
\begin{equation}
  \zz = \frac{\xx}{\sigmain} + \sigma \noise
  \text{,}
\end{equation}

From which it follows that 
\begin{equation}
  \xx = \frac{\zz - \frac{\sigmanoise}{\sigmadata^2}\vv}{\frac{1}{\sigmain} + \frac{\sigmanoise^2}{\sigmadata^2}}
  \text{,}
\end{equation}

And consequently
\begin{equation}
  \vv = \frac{\sigmadata^2 \zz - (\frac{\sigmadata^2}{\sigmain} + \sigmadata^2) \xx}{\sigmanoise}
  \text{,}
\end{equation}

We can use this definition to define our loss and find the training weight
\begin{eqnarray}
  \mathcal{L}(\netd) &=& \mathbb{E}_{\sigmanoise \sim \ptrain} \big[ \lossweight(\sigmanoise) ~\mathcal{L}(\netd; \sigmanoise) \big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lossweight(\sigmanoise) ~\big\lVert \netd(\frac{\xx}{\sigmain} + \sigmanoise \noise; \sigmanoise) - \vv \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lossweight(\sigmanoise) ~\big\lVert \vvh - \vv \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lossweight(\sigmanoise) ~\big\lVert \frac{\sigmadata^2 \zz - (\frac{\sigmadata^2}{\sigmain} + \sigmadata^2) \xxh}{\sigmanoise} - \frac{\sigmadata^2 \zz - (\frac{\sigmadata^2}{\sigmain} + \sigmadata^2) \xx}{\sigmanoise} \big\rVert^2_2 \Big] \\
  &=& \mathbb{E}_{\sigmanoise, \xx, \noise} \Big[ \lossweight(\sigmanoise) \frac{(\frac{\sigmadata^2}{\sigmain} + \sigmanoise^2)^2}{\sigmanoise^2} ~\big\lVert \xxh - \xx \big\rVert^2_2 \Big] \\
  \text{,}
\end{eqnarray}

We recover the same loss weighting as EDM by imposing that the effective loss weight equals the EDM one
\begin{eqnarray}
 \lossweight(\sigmanoise) \frac{(\frac{\sigmadata^2}{\sigmain} + \sigmanoise^2)^2}{\sigmanoise^2} &=& \frac{1}{\sigmadata^2} + \frac{1}{\sigmanoise^2} \\
  \lossweight(\sigmanoise) &=& \frac{\sigmanoise^2 + \sigmadata^2}{\sigmadata^2 (\frac{\sigmadata^2}{\sigmain} + \sigmanoise^2)^2}
  \text{,}
\end{eqnarray}
